A gradient boosting approach for optimal selection of bidding strategies in reservoir hydro

Power producers use a wide range of decision support systems to manage and plan for sales in the day-ahead electricity market, and they are often faced with the challenge of choosing the most advantageous bidding strategy for any given day. The optimal solution is not known until after spot clearing. Results from the models and strategy used, and their impact on profitability, can either continuously be registered, or simulated with use of historic data. Access to an increasing amount of data opens for the application of machine learning models to predict the best combination of models and strategy for any given day. In this article, historical performance of two given bidding strategies over several years have been analyzed with a combination of domain knowledge and machine learning techniques (gradient boosting and neural networks). A wide range of variables accessible to the models prior to bidding have been evaluated to predict the optimal strategy for a given day. Results indicate that a machine learning model can learn to slightly outperform a static strategy where one bidding method is chosen based on overall historic performance.

==> fig_strategygap.tex <==
\begin{tikzpicture}[scale=0.7] %[x={10.0pt},y={10.0pt}]

\definecolor{color0}{rgb}{0.886274509803922,0.290196078431373,0.2}
\definecolor{color1}{rgb}{0.203921568627451,0.541176470588235,0.741176470588235}

\begin{axis}[
axis background/.style={fill=white!89.80392156862746!black},
axis line style={white},
tick align=outside,
tick pos=left,
x grid style={white},
xlabel={\hspace{1cm} 2016 \hspace{1cm} 2017 \hspace{1cm} 2018},
xmajorgrids,
xmin=32.3743576649837, xmax=1131.62564233502,
xtick style={color=white!33.33333333333333!black},
xtick={46,137,228,319,410,501,592,683,774,865,956,1047},
xticklabels={Q1,Q2,Q3,Q4,Q1,Q2,Q3,Q4,Q1,Q2,Q3,Q4},
y grid style={white},
ylabel={delta stoch-determ},
ymajorgrids,
ymin=-927.33566049903, ymax=637.654650788729,
ytick style={color=white!33.33333333333333!black}
]
\addplot [only marks, draw=color0, fill=color0, colormap/viridis, mark=triangle]
table{%
x                      y
92 -257.875070800015
93 -260.561137215991
94 -282.129465617007
95 -280.545974295004
96 -260.75491407502
97 -211.506476572016
98 -204.139832704008
99 -295.650457597978
100 -333.835715126974
101 -315.099640954984
102 -375.681863197999
103 -444.657081988989
104 -357.918570437992
105 -353.651192144986
106 -377.146097371005
107 -317.798832656001
108 -324.694412351004
109 -335.330111013987
110 -531.12324371899
111 -481.270371158025
112 -577.73892427102
113 -562.048840303003
114 -206.282803909009
115 -232.121295196994
117 -425.812026701984
122 -340.363439626992
123 -230.198967525008
124 -264.613664523989
125 -237.201228432008
127 -483.073800673999
128 -336.335813374026
129 -373.453052675992
131 -283.73945582303
132 -820.667450757988
133 -718.747880231007
134 -479.958407763042
135 -468.118270367966
136 -484.953870457015
137 -322.357759331993
138 -415.779438488011
139 -362.785854814021
141 -475.154482961982
142 -325.744544422021
143 -267.521491640015
145 -212.845015589992
146 -272.065891378996
147 -269.35682210201
178 -216.982559357013
484 -210.903370468994
489 -401.531590572908
492 -778.553149924963
495 -516.437586341985
503 201.983585898997
505 207.307050698088
508 -306.361557638971
541 219.707793697016
551 271.385587650002
559 -296.017647241941
562 239.72012207401
563 285.929042239906
565 -243.31540622504
566 -303.594126498909
627 -291.006607678995
628 -305.805790787999
643 -218.305437737959
647 -220.346136491979
713 294.841672309907
714 447.124688970158
715 278.837794590043
718 543.142418029951
817 -217.577524413937
833 -358.104388464999
834 -420.390050846006
835 -685.25304943099
838 -452.119990483974
839 -456.204328951018
844 -529.364049326017
845 -344.637169338006
846 -492.009317752003
879 -591.68921252992
881 359.078451900044
902 -273.684777989984
928 385.138098999858
940 -202.773311109981
951 -281.704174100189
970 -452.563252130058
972 -758.363771270029
974 -254.812795300037
975 241.837399049895
979 295.596213479992
992 -571.564178830013
993 -835.243381279986
994 -211.668802289758
995 -319.827704799827
997 248.866492229979
998 268.83378928015
1002 326.852525069844
1027 238.877984859981
1029 307.16823571967
1064 272.529102829751
1069 545.562371569686
1071 210.163856029976
1072 344.644401179627
};
\end{axis}
        \node [below=1cm, align=right,text width=5cm]
        {\tiny
            b) Strategy gap with threshold 2016-2018
        };
\end{tikzpicture}


==> fig_variableReduction.tex <==
\begin{tikzpicture}[scale=0.7]

\definecolor{color0}{rgb}{0.886274509803922,0.290196078431373,0.2}
\definecolor{color1}{rgb}{0.203921568627451,0.541176470588235,0.741176470588235}

\begin{axis}[
axis background/.style={fill=white!89.80392156862746!black},
axis line style={white},
legend cell align={left},
legend style={draw=white!80.0!black, fill=white!89.80392156862746!black},
tick align=outside,
tick pos=left,
x grid style={white},
xlabel={number of variables dropped},
xmajorgrids,
xmin=-0.35, xmax=7.35,
xtick style={color=white!33.33333333333333!black},
y grid style={white},
ymajorgrids,
ymin=0.911516853932584, ymax=1.00421348314607,
ytick style={color=white!33.33333333333333!black}
]
\addplot [semithick, color0]
table {%
0 0.915730337078652
1 0.932584269662921
2 0.932584269662921
3 0.966292134831461
4 0.966292134831461
5 1
6 0.938202247191011
7 0.932584269662921
};
\addlegendentry{accuracy}
\addplot [semithick, color1]
table {%
0 0.998225239787168
1 0.980928447835657
2 1
3 0.952879848805052
4 0.942633844849395
5 0.954362575823055
6 0.974990666480136
7 0.982570021007104
};
\addlegendentry{performance}
\end{axis}
        \node [below=1cm, align=right,text width=5cm]
        {\tiny
            b) Accuracy and performance after variable reduction 
        };
\end{tikzpicture}
\qquad
% This file was created by matplotlib2tikz v0.7.5.
\begin{tikzpicture}[scale=0.7]

\definecolor{color0}{rgb}{0.886274509803922,0.290196078431373,0.2}

\begin{axis}[
axis background/.style={fill=white!89.80392156862746!black},
axis line style={white},
tick align=outside,
tick pos=left,
title={Feature importance},
x grid style={white},
xlabel={F score},
xmajorgrids,
xmin=0, xmax=6.0946946935156,
xtick style={color=white!33.33333333333333!black},
y grid style={white},
ylabel={Features},
ymajorgrids,
ymin=-1, ymax=8,
ytick style={color=white!33.33333333333333!black},
ytick={0,1,2,3,4,5,6,7},
yticklabels={vol\_p,vol\_prog,reservoir\_filling\_2,reservoir\_filling\_1,average\_p,average\_prog,inflow\_deviation,water\_value}
]
\draw[fill=color0,draw opacity=0,very thin] (axis cs:0,-0.1) rectangle (axis cs:1.87865641817283,0.1);
\draw[fill=color0,draw opacity=0,very thin] (axis cs:0,0.9) rectangle (axis cs:1.91402470495283,1.1);
\draw[fill=color0,draw opacity=0,very thin] (axis cs:0,1.9) rectangle (axis cs:1.97060569318812,2.1);
\draw[fill=color0,draw opacity=0,very thin] (axis cs:0,2.9) rectangle (axis cs:2.152042679408,3.1);
\draw[fill=color0,draw opacity=0,very thin] (axis cs:0,3.9) rectangle (axis cs:2.25784053455556,4.1);
\draw[fill=color0,draw opacity=0,very thin] (axis cs:0,4.9) rectangle (axis cs:2.28897621048113,5.1);
\draw[fill=color0,draw opacity=0,very thin] (axis cs:0,5.9) rectangle (axis cs:3.64748083685366,6.1);
\draw[fill=color0,draw opacity=0,very thin] (axis cs:0,6.9) rectangle (axis cs:5.54063153955963,7.1);
\addplot [ultra thick, red, dashed]
table {%
2.28897621048113 -1
2.28897621048113 8
};
\end{axis}
        \node [below=1cm, align=right,text width=5cm]
        {\tiny
            b) Feature selection based on GAIN and threshold
        };

\end{tikzpicture}
